SIR-Hawkes: Linking Epidemic Models and Hawkes Processes to Model Diffusions in Finite Populations

Among the statistical tools for online information diffusion modeling, both epidemic models and Hawkes point processes are popular choices. The former originate from epidemiology, and consider information as a viral contagion which spreads into a population of online users. The latter have roots in geophysics and finance, view individual actions as discrete events in continuous time, and modulate the rate of events according to the self-exciting nature of event sequences. Here, we establish a novel connection between these two frameworks. Namely, the rate of events in an extended Hawkes model is identical to the rate of new infections in the Susceptible-Infected-Recovered (SIR) model after marginalizing out recovery events -- which are unobserved in a Hawkes process. This result paves the way to apply tools developed for SIR to Hawkes, and vice versa. It also leads to HawkesN, a generalization of the Hawkes model which accounts for a finite population size. Finally, we derive the distribution of cascade sizes for HawkesN, inspired by methods in stochastic SIR. Such distributions provide nuanced explanations to the general unpredictability of popularity: the distribution for diffusion cascade sizes tends to have two modes, one corresponding to large cascade sizes and another one around zero.

==> journal-extension-future-work.tex <==
%!TEX root = sir-hawkes.tex

\section{Journal extension and future work material}

The material in the following sections is either intended for the planned journal extension (shorter term) or longer term future work.
The journal paper will have the narrative structure differently from the conference paper:
the conference article proposes HawkesN (a new diffusion model) -> links HawkesN to the SIR -> applies SIR specific tools to get a distribution of cascade size;
the journal paper will concentrate on the equivalence (in expectation) between the two classes of models, will deal with SIS, will discuss $R0$ vs $n^\ast$ and introduce new tools such as diffusion speed and duration.

\subsection{SIR corresponding to HawkesN with power-law kernel}

We can show that the Hawkes process and the SIR model are equivalent when the kernel function of the Hawkes process is the complementary cumulative density function (CCDF) of the distribution of recovery times for the SIR model.

\TODO{MAR}{This came from the HawkesN section.}
\textbf{Equivalence with the basic SIR model.}
The \texttt{HawkesN} model is mathematically equivalent with the basic SIR model (with finite population $N$), for $\mu(t) = 0, \forall t \geq 0$.
More generally we have the relationship between the \texttt{HawkesN} process and variations on the basic SIR compartmental model, that the kernel of the Hawkes process corresponds to the complementary CDF of the time-to-recovery distribution of the SIR model, i.e. $\phi(\Delta t) = 1-cdf(\Delta t)$. In the case of a power law kernel, the pdf of the recovery time would also be a power law (Pareto) distribution. 

\textbf{From newly infected individuals to events in Hawkes.}
Note that in the equivalent Hawkes process, events corresponds to new infected individuals.
In most application, what we observe are the actions of infected individuals (i.e. tweets, views of a video, resharing of a news item).
Most often the infection (or how information spreads spreads from use to user) is not observed.
One can pass from the infected users Hawkes process to the actions Hawkes process by using the clustering property of Poisson processes: if in a Poisson process we replace individual events with entire clusters of events generated through a Poisson process, the resulted point process is a Poisson process.
Each infected user emits actions as a Poisson process.
Replacing each infected user in the user Hawkes process with its sequence of actions results the observed event point process.

\subsection{SIS Model}

\TODO{MAR}{Journal extension -- this would go well with a more detailed linking analysis.}

We now repeat the analysis for the simple SIS Model (with no recovered/immune state) since that too may be a good model for modeling online user interest. In an SIS Model, there is no recovered (a.k.a. ``immune'') state. Instead individuals recovering from the infection simply return to the susceptible state, allowing the outbreak to continue and individuals to become infected multiple times over:
\begin{eqnarray}
\frac{dS(t)}{dt} &=& -\beta \frac{S(t)}{N}I(t) + \gamma I(t)\\
\frac{dI(t)}{dt} &=& \beta \frac{S(t)}{N}I(t) - \gamma I(t) \label{eq:sis-di}
\end{eqnarray}

This type of model where people can return to a susceptible state should make for a very interesting further extension on the Hawkes process, since it allows us to build an extension on the Hawkes process where the population is finite, but the self-exciting nature doesn't tend to die out after a certain amount of time.

Under this model, the rate of \emph{new infections} at time $t$ is the same as for the SIR model:
\begin{eqnarray}
\lambda(t) &=& \beta S(t)I(t) \\
		   &=& -\frac{dS(t)}{dt} + \gamma I(t)
\end{eqnarray}
The additional term on the right side of the equation complicates the equation for the susceptible population at time $t$, causing it to become recursive:
\begin{eqnarray}
	S(t) &=& S(0) + \int_{0}^{t}\frac{dS(t)}{dt} dt \\
		 &=& S(0) - \int_{0}^{t} \lambda(t) dt + \gamma \int_{0}^{t} I(t) dt \\
		 &=& S(0) - \int_{0}^{t} \lambda(t) dt + \gamma \int_{0}^{t} \frac{\lambda(t)}{\beta S(t)} dt \\
		 &=& S(0) - \int_{0}^{t} \lambda(t)[1 - \frac{1}{R_0 S(t)}] dt 
\end{eqnarray}

\TODO{MAR}{While this is a self-consistent equation, it helps to notice that when $N \rightarrow \infty$, SIR and SIS are equivalent. This is because $S(t) \rightarrow \infty, \frac{S(t)}{N} \rightarrow 1, \forall t \geq 0$. This renders both Eq.~\eqref{eq:sir-di} and \eqref{eq:sis-di} to: }
\begin{equation}
	\frac{dI(t)}{dt} = I(t) (\beta - \gamma)
\end{equation}

\TODO{MAR}{In other words, both SIS and SIR are equivalent to Hawkes under infinite population assumption.}

\subsection{SIR Model with Exogenous Seed Function}

If the background intensity $\mu(t)$ for the Hawkes model in Eq.~\eqref{eq:phi-hawkes} is not set to zero (for the equivalence mapping given in Theorem~\ref{theorem:expected-equivalence}), then the corresponding SIR model would require an additional ``background infection rate'' or ``seeding intensity'' term within Eq.~\eqref{eq:sir-di}: 
\begin{eqnarray}
	\frac{dI(t)}{dt} &=& \mu(t) + \beta \frac{S(t)}{N} I(t) - \gamma I(t) \label{eq:sir-di+mu} 
\end{eqnarray}
This model provides an alternative approach to drive an epidemic model with an external influence with respect to more common mechanism to make the parameter $\beta$ time dependent. The latter is commonly used to add seasonal effects to an epidemic model [CITATION NEEDED].

\subsection{Branching factor, Basic Reproduction number and speed of diffusion}

\TODO{MAR}{I think this is linked intimately to the speed of unfolding of the cascade.}

The branching factor (or the branching ratio) in a Hawkes process is defined as the expected (mean) number of offspring events generated by a single event:
\begin{equation}
	n^* = \int_0^\infty \phi(\tau) d\tau \enspace.
\end{equation}
It is known~\cite{Helmstetter2002} that the branching factor is an indicator of the total size of the endogenous reaction in a Hawkes self-exciting process.
When $n^* < 1$, the process is in a \emph{sub-critical} regime, in which each event spawns, in average, less than one offspring.
The event intensity eventually converges to zero and the process dies out.
When $n^* > 1$ we have a \emph{super-critical} regime, in which each events spawns more than an offspring.
In turn, this leads to an exponential increase in the event intensity.
Considering that in the classic Hawkes process, there is no upper bound on the number of events, a super-critical regime leads to an infinite number of events in the Hawkes process.
For a Hawkes process with an exponential decaying kernel, the branching factor can be calculated as:
\begin{equation}
	n^* = \int_0^\infty \phi(\tau) d\tau = \int_0^\infty \beta e^{- \gamma \tau} = \frac{\beta}{\gamma}
\end{equation}
When we are considering events in the Hawkes model to be \textbf{new infections} in the SIR model, then $n^*$ is equivalent to the basic reproduction number $R_0$, defined in Sec.~\ref{subsec:sir-model}.

\TODO{@}{Questions:
We need to discuss further thresholds for $R_0$ that determine whether the outbreak will become endemic in the population or not.
A comparative sub-/super-  criticality discussion between $n^*$ and $R_0$ seems also needed.}

\textbf{Temporal Reproduction Number}
The Basic Reproduction Number was defined as the expected number of secondary infections caused by the initial infection seed, early on in the outbreak.
As the epidemic progresses, the number of susceptible individuals decreases.
We define the Temporal Reproduction Number $R_{t_i}$ as the expected number of new infections generated by a single infected individual, who got infected at time $t_i$ in the epidemic.
$R_{t_i}$ is shown in Fig.~\ref{fig:example-phi-Hawkes-SIR} (right) and it can be computed as the area under $\phi^S_{t_i}(t)$ (and observing that $\phi^S_{t_i}(t) = 0, \forall t < t_i$):
\begin{align}
	R_{t_i} &= \int_0^\infty \phi^S_{t_i}(t) dt = \int_0^{t_i} \phi^S_{t_i}(t) dt + \int_{t_i}^\infty \beta \frac{S(t)}{N}e^{-\gamma (t - t_i)} dt \nonumber \\
	&\overset{x = t-t_i}{=} \int_0^\infty \beta \frac{S(x + t_i)}{N}e^{-\gamma x} dx
\end{align}
\TODO{MAR}{But unfortunately, no closed form as far as I can see. @mark? 
I believe it would be valuable to analyze the $R_{t_i}$ over time, or the virulence of the epidemic with time.}

\subsection{Population Dynamics in SIR: Births and Deaths}

An SIR model with births (i.e. where there is a non-static, growing population $N(t)$) may also be an interesting model that allows for good models of online user behaviour, where the self-exciting process doesn't die out after a period of time. -- A simple model here would allow the population to grow at a constant rate: $N(t) = N(t_0) + m(t - t_0)$.

\TODO{MAR}{How about using a custom made $\mu(t)$ to deal with dynamics?}

\subsection{Long derivation of the equivalence SIR-HawkesN}

\TODO{MAR}{This is the first draft of the derivation, that goes through the bivariate Poisson process. It will be shortened in the paper, saving it here.}

\textbf{SIR as a Bivariate Markov Chain}
One classic view of the SIR model is that of a bivariate continuous time-homogeneous Markov chain $\{S(t), I(t)\}$ as described in \citet{Allen2008}.
In other words, $S(t)$ and $I(t)$ uniquely define the state of the process, with $R(t) = N - S(t) - I(t)$ for a fixed population.
Given a state $\{S(t)= s, I(t)= i\}$ at time $t$, in the infinitesimal interval $\delta t$, one of the following three options can happen 
($\delta t$ is chosen small enough to guarantee that at most one event occurs between $t$ and $t + \delta t$):
a new infection occurs and the system transitions to the state $\{S(t + \delta t)= s - 1, I(t + \delta t)= i + 1\}$;
a new recovery occurs and the system transitions to the state $\{S(t + \delta t)= s, I(t + \delta t) = i - 1\}$;
or 
none of the above happen and the system remains in the state $\{S(t + \delta t) = s, I(t + \delta t) = i\}$.

Considering $R(t)$ as the number of recovered individuals at time $t$ and $C(t)= I(t)+ R(t)$ as the total number of infections %infected individuals 
by time $t$, \citet{Yan2008} shows that $\{R(t)\}$ and $\{C(t)\}$ are also stochastic processes. 
In addition, given $\mathcal{H}_t$ the history of the epidemic process up to time $t$ and under the time stationary Markov chain assumption, \citet{Yan2008} computes the transition probabilities at time $t$:
\begin{equation} \label{eq:transition-bivariate-Poisson}
\left\{
	\begin{array}{ll}
		\mathbbm{P}(\delta C(t) = 1, \delta R(t) = 0 | \mathcal{H}_t) \approx \beta \frac{S(t)}{N}I(t)\delta t \enspace, \\
		\mathbbm{P}(\delta C(t) = 0, \delta R(t) = 1 |\mathcal{H}_t) \approx \gamma I(t)\delta t \enspace, \\
		\mathbbm{P}(\delta C(t) = 0, \delta R(t) = 0 |\mathcal{H}_t) \approx 1 - \beta \frac{S(t)}{N}I(t)\delta t - \gamma I(t)\delta t. \\
	\end{array}
\right.
\end{equation}

\textbf{SIR as a Bivariate Point Process.}
This leads us to state the following lemma:
\begin{lemma} \label{lemma:SIR-bivariate-poisson}
	The SIR process can be represented as a bivariate point process, in which two types of events occur: \emph{infection events} and \emph{recovery events}.
	The $j$-th infected individual in the SIR process gets infected at time $t^i_j$ and recovers at time $t^r_j$.
	Her time to recovery is defined as: $\tau_j = t^r_j - t^i_j$.
\end{lemma}

\emph{Proof:} 
Let $C_t$ be the counting process of the \emph{infection process} and $R_t$ the counting process of the \emph{recovery process}.
%Visibly, the 
The SIR model is completely specified %using 
by $C_t$ and $R_t$: 
$S(t) = N - C_t$, $I(t) = C_t - R_t$ and $R(t) = R_t$.
%Note that, without loss of generality, we have assigned ids to individuals based on the order they get infected\footnote{Note that not all $N$ individuals need to get infected in an SIR epidemic~\cite{Allen2008}, i.e. $S(\infty) \geq 0$.}.
Fig.~\ref{fig:sir-two-processes} illustrates an SIR as a bivariate Poisson process: 
five infection events occur at times $t^i_1,.., t^i_5$ (shown in red);
five recovery events occur at $t^r_1, ..t^r_5$ (shown in blue).
To each infection event corresponds a recovery event.
The middle panel of Fig.~\ref{fig:sir-two-processes} show the size of the infected population $I(t)$ over time.
Each new infection event increments $I(t)$, and each new recovery decreases $I(t)$ by one.

\textbf{Intensity View of the SIR Process.}
Next we compute the intensity of each of the Poisson processes defined here above.
Given how $\delta t$ is chosen (Eq.~\eqref{eq:transition-bivariate-Poisson}, \citep{Allen2008,Yan2008}) -- i.e. small enough to guarantee the occurrence of a single event --, the following holds:
\begin{equation} \label{eq:transition-bivariate-Poisson-extra}
	\mathbbm{P}(\delta C(t) = 1, \delta R(t) = 1 | \mathcal{H}_t) = 0
\end{equation}
Using the marginal property and Eq.~\eqref{eq:transition-bivariate-Poisson} and ~\eqref{eq:transition-bivariate-Poisson-extra}, we obtain: \nb{\rvx{MC: Two different notations $C_t$ and $C(t)$ used to denote the same process. Not really much of a problem though ...}}
\begin{align}
	\mathbbm{P}(C_{t+\delta t} - C_t &= 1 | \mathcal{H}_t) = \mathbbm{P}(\delta C(t) = 1, \delta R(t) = 0 | \mathcal{H}_t) \nonumber \\ 
	&+ \mathbbm{P}(\delta C(t) = 1, \delta R(t) = 1 | \mathcal{H}_t) \approx \beta \frac{S(t)}{N}I(t)\delta t \nonumber \\
	\mathbbm{P}(C_{t+\delta t} - C_t & > 1 | \mathcal{H}_t) = 0 \nonumber \\
	\mathbbm{P}(C_{t+\delta t} - C_t &= 0 | \mathcal{H}_t) \approx 1 - \beta \frac{S(t)}{N}I(t)\delta t.    \label{eq:intesity-Ct}
\end{align} 
Given Lemma~\ref{lemma:SIR-bivariate-poisson}, Eq~\eqref{eq:intesity-Ct} and the definition of a non-homogeneous Poisson process (Eq.~\eqref{eq:non-homog-poisson}), we have proven the following lemma:
\begin{lemma}\label{eq:lambda-SIR-definition}
	An SIR process can be formulated as a bivariate non-homogeneous Poisson process, in which the \emph{new infection rate} $\lambda^I(t)$ and the \emph{new recovery rate} $\lambda^R(t)$ have the following formulations:
	\begin{equation*} 
		\lambda^I(t) = \beta \frac{S(t)}{N} I(t) ; \; \lambda^R(t) = \gamma I(t).
	\end{equation*}
\end{lemma}

The bottom panel of Fig.~\ref{fig:sir-two-processes} shows the new infection and new recovery rates for the SIR process with five individuals.
At first, both $\lambda^I(t)$ and $\lambda^R(t)$ are following closely $I(t)$, with the infection rate significantly higher than the recovery rate -- this is SIR's incipient phase of exploding number of infections.
As the the number of susceptible individuals $S(t)$ gets depleted, the $\frac{S(t)}{N}$ term draws down $\lambda^I(t)$ which becomes zero after the fifth infection ($S(t) = 0, t \geq t^i_5$).
The new recovery rate also becomes null after the last infected individual recovers ($I(t) = 0, t \geq t^r_5$).

\textbf{Exciting vs. Inhibiting Process.}
Applying the definition of the counting process~\cite{Rizoiu2017a}, we obtain $C_t = \sum_{j \geq 1} \mathbbm{1}(t^i_j < t)$ and $R_t = \sum_{j \geq 1} \mathbbm{1}(t^r_j < t)$.
$\mathbbm{1}(\cdot)$ is the indicator function equal to 1 if the condition is true, zero otherwise.
Given that $I(t) = C_t - R_t$, we obtain:\nb{\rvx{MC: I didn't follow the derivation 100\%. Can you add an extra step?}}
\begin{equation}
	\lambda^I(t) = \textcolor{blue}{\sum_{t^i_j < t} \beta \frac{S(t)}{N}} - \textcolor{red}{\sum_{t^r_j < t} \beta \frac{S(t)}{N}} ; \; \lambda^R(t) = \textcolor{blue}{\sum_{t^i_j < t} \gamma} - \textcolor{red}{\sum_{t^r_j < t} \gamma},
\end{equation}
where we separated in blue the contributions of the infection events and in red the contributions of the recovery events.
Visibly, each infection event increases both new infection rate $\lambda^I(t)$ and the new recovery rate $\lambda^R(t)$.
Each recovery event decreases both rates.
The infection process is an \emph{exciting process} (the occurrence of an infection increases the likelihood of other infections and recoveries), while the recovery process is an \emph{inhibiting process}.
This behavior can also be observed in Fig.~\ref{fig:sir-two-processes}.

\textbf{The expected new infections rate.}
When linking SIR and HawkesN, we consider each new infection in SIR as an event in HawkesN.
The new recovery events are unobserved in HawkesN.
Therefore, we compute the expected rate of new infections, averaging over the time to recovery -- i.e. $\mathbbm{E}_\tau[\lambda^I(t)]$ in Theorem~\ref{theorem:expected-equivalence}:
\begin{align}
	\mathbbm{E}_{\tau_j} \left[ \lambda^I(t) \right] 
	&= \mathbbm{E}_{\tau_j} \left[ \beta \frac{S(t)}{N} \sum_{t^i_j < t} \mathbbm{1}(t^i_j + \tau_j > t) \right] \nonumber \\
	&= \sum_{t^i_j < t} \mathbbm{E}_{\tau_j} \left[ \beta \frac{S(t)}{N} \mathbbm{1}(t^i_j + \tau_j > t) \right] \nonumber \\
	&= \sum_{t^i_j < t}  \int_{0}^{\infty}\beta \frac{S(t)}{N} \mathbbm{1}(t^i_j + \tau > t) r(\tau) d\tau \nonumber \\
	&= \sum_{t^i_j < t}  \beta \frac{S(t)}{N} \int_{t-t^i_j}^{\infty} r(\tau) d\tau , \label{eq:exp-lambda-i}
\end{align}
where $r(\tau)$ is the probability distribution function for the time to recovery.
Knowing that $\tau_j$ are exponentially distributed with parameter $\gamma$ and that $S(t) = N - C_t$, we obtain:
\begin{equation} \label{eq:SIR-expectation}
	\mathbbm{E}_{\tau_j} \left[ \lambda^I(t) \right]  = \left(1 - \frac{C_t}{N} \right) \sum_{t^i_j < t} \beta e^{-\gamma (t - t^i_j)} 
\end{equation}


\textbf{Expected event rate in HawkesN over user influence.}
In the stochastic SIR model, the actions of each individual are guided by the same set of global rules, i.e. the differences between individuals are not observed.
The HawkesN model with the kernel defined in Eq.~\eqref{eq:kernel-function-hawkesN} accounts for different local user influences, which are averaged out in Theorem~\ref{theorem:expected-equivalence}. 
%the local user influence in  before linking HawkesN to SIR.
We obtain:
\begin{align} \label{eq:HawkesN-expectation}
	\mathbbm{E}_m\left[\lambda^H(t)\right]
		&= \mathbbm{E}_m\left[ \left( 1 - \frac{N_t}{N} \right) \left( \mu(t) + \sum_{t_j < t} \kappa m^\eta_j \theta e^{-\theta (t - t_j)} \right) \right] \nonumber \\
		&=  \left( 1 - \frac{N_t}{N} \right) \left( \mu(t) + \sum_{t_j < t} \kappa  \theta e^{-\theta (t - t_j)} \int_1^\infty m^\eta p(m) dm \right) \nonumber \\
		&=  \left( 1 - \frac{N_t}{N} \right) \left( \mu(t) + \sum_{t_j < t} K  \theta e^{-\theta (t - t_j)} \right)
\end{align}
\citet{Mishra2016} have studied the distribution of local user influence in a large sample of tweets, and they found it to be a power-law of exponent $\alpha = 2.016$.
As a result, $K$ in Eq.~\eqref{eq:HawkesN-expectation} is $K = \kappa \frac{\alpha - 1}{\alpha - \eta - 1}$. 
\nb{\rvx{MC: Should we note that the same "local user influence" effect could be achieved in the SIR model by making the interaction rate $\epsilon$ and/or the transmission probability $\rho$ user dependent?}}

%Finally, from Eq.~\eqref{eq:SIR-expectation} and~\eqref{eq:HawkesN-expectation}, we obtain the following corollary to Theorem~\ref{theorem:expected-equivalence}:
%\begin{corollary} \label{corollary:equivalence}
%	An SIR process of parameters $\beta$ and $\gamma$ has an equivalent (in expectation) HawkesN process of parameters $\kappa, \eta$ and $\theta$ so that
%	\begin{equation*}
%		\mathbbm{E}_{\tau_j} \left[ \lambda^I(t) \right] = \mathbbm{E}_m\left[\lambda^H(t)\right], \forall t \geq 0,
%	\end{equation*}
%	when $\mu(t) = 0, N_t = C_t, \beta = \kappa \theta \frac{\alpha - 1}{\alpha - \eta - 1}, \gamma = \theta$ .
%\end{corollary}
We can see that Eq.~\eqref{eq:SIR-expectation} and~\eqref{eq:HawkesN-expectation} are identical when $N_t = C_t$ (i.e. we observed the same random process) and under the parameter equivalence in Theorem~\ref{theorem:expected-equivalence}.
That is to say, the new infection point process in an SIR model is equivalent in expectation with a HawkesN point-process with no background event rate.
This completes the proof of Theorem~\ref{theorem:expected-equivalence}.


%\subsection{Notes}
%
%Note that on the Wikipedia page for epidemic models \url{https://en.wikipedia.org/wiki/Epidemic_model#The_SIS_model_with_births_and_deaths} the equations for the SIR model define $\beta$ differently, using a denominator of $N$ in the equation for $\frac{dS(t)}{dt}=-\beta \frac{S(t)I(t)}{N}$ Defining things in this way may simplify the derivation above. It may also simplify the births/deaths models.

